ReasonPix2Pix: Instruction Reasoning Dataset for Advanced Image Editing

Instruction-based image editing focuses on equipping a generative model with the capacity to adhere to human-written instructions for editing images. Current approaches typically comprehend explicit and specific instructions. However, they often exhibit a deficiency in executing active reasoning capacities required to comprehend instructions that are implicit or insufficiently defined. To enhance active reasoning capabilities and impart intelligence to the editing model, we introduce ReasonPix2Pix, a comprehensive reasoning-attentive instruction editing dataset. The dataset is characterized by 1) reasoning instruction, 2) more realistic images from fine-grained categories, and 3) increased variances between input and edited images. When fine-tuned with our dataset under supervised conditions, the model demonstrates superior performance in instructional editing tasks, independent of whether the tasks require reasoning or not. The code will be available at https://github.com/Jin-Ying/ReasonPix2Pix.

==> sec/intro.tex <==

\begin{comment}
    \section{Introduction}
\label{sec:intro}

Instruction-based image editing aims at training a generative model that edits images according to instructions. Concretely, the model takes one input image and one text instruction about how to edit the image and then produces the edited image. The instructions point to the modifications made to input images, instead of the captions of target images. The lack of information in the instructions makes it more challenging than text-to-image generation tasks. 

Previous methods, \eg InstructPix2Pix, produce a large-scale paired dataset with large language model~\misscite{} and text-to-image model~\misscite{}. With this dataset that captures the interactive knowledge between language and image pairs, these methods are proven to be effective, generating numerous high-quality results. However, its ability to understand instructions is still quite limited. 

First, incorporating a text encoder such as CLIP to absorb text information, previous methods are incapable of understanding instructions as a sentence rather than words. Take InstructPix2Pix as an instance, as shown in Figure~\ref{fig:pearl-mistake}, when facing the instruction 'add a pair of sunglasses', the model produces reasonable output (\ie a woman wearing sunglasses). However, if we alter the instruction to the opposite meaning, 'she prefers face mask to sunglasses', the model generates similar results, which is absolutely wrong. Why? The model is only supervised by the word 'sunglasses' instead of understanding the instruction as a whole sentence. 

Next, previous methods never gain the reasoning ability towards instructions. For example, InstructPix2Pix can tackle 'replace the fruits with a cake', but it is ignorant of instructions such as 'today is her birthday', incapable of editing the image accordingly. Therefore, we target injecting reasoning ability into instruction-based image editing models. An intuitive solution is to utilize language models to produce reasoning results. However, in instruction-based image editing, the understanding of instructions is not confined to text modality. As shown in Figure~\ref{fig:50-years}, given the instruction 'make it 50 years later', the model can edit the beautiful young woman to an old one, but it can not tackle objects such as apples. In addition, for a statue, it is unreasonable that it becomes an old man after 50 years. The reasonable results may be 1) for a young woman, she will become old, 2) for an apple, it will rot, 3) for a statue, it may be broken. We can observe that with the same instruction, we shall produce different results according to different images. Therefore, the model must take both input image and instruction into consideration. 

Towards the aforementioned challenges, we construct a large-scale dataset, with paired images and reasoning instructions. Compared with previous typical datasets, our dataset contains 1) in-direct yet adequate instructions to empower model reasoning ability, 2) large amounts of real images from fine-grained categories, and 3) more variations between input and edited images, especially at the geometry level. 

With this carefully designed dataset, we train an instruction-based editing model that seamlessly incorporates multi-modal language knowledge into generative models. Our model shows reasoning ability to instructions, making instruction-based image editing more practical. With the help of our high-quality dataset, our model also shows stronger generative ability.

\end{comment}

\section{Introduction}
\label{sec:intro}
%Instruction-based image editing aims to teach a generative model to follow human-written instructions for image editing. It makes the AIGC system to understand the explicit and specific instruction of human, such as \textit{replace the fruits with cake}. However, current instruction-based image editing models lack reasoning ability to understand or analysis the indirect and vague instructions. For examples, instruction \textit{make the room tidy} should be analyzed and decomposed to many explicit and specific instructions \textit{replace loose clothing with neatly folded clothing, remove trash from the floor, make the bed smooth}, instruction \textit{let her be in ancient times} should be analyzed and decomposed to instructions \textit{change the background to an ancient style, replace her costume with ancient costume}. Such self-reasoning ability helps the AIGC system understand the intent of the huaman and is crucial in developing next-generation intelligent AIGC systems
Instruction-based image editing aims at furnishing a generative model with the capacity to adhere to human-written instructions for editing images, which is vital to facilitate the AI-Generated Content (AIGC) system’s comprehension of human intentions.  

Prevailing instruction-based image editing frameworks typically comprehend explicit and specific instructions, such as \textit{``replace the fruits with cake"}. 
Unfortunately, these models display a deficiency in active reasoning capabilities, specifically lacking the capacity to comprehend implicit or inadequately defined instructions. 
This requires manual intervention to either make implicit instructions explicit or deconstruct the instructions into multiple explicit, specific instructions to align with the capabilities of these models. 
For examples, the instruction \textit{``make the room tidy"} necessitates manual partitioning into various steps such as \textit{``replace loose clothing with neatly folded clothing"}, \textit{``remove garbage from the floor"}, and \textit{``smooth the bed linens"}, among others. 
Similarly, the implicit instruction \textit{``she is the star of the show"} necessitates human intervention to render it explicit as \textit{``add some sparkles and a spotlight effect to the image"}.
%Similarly, the instruction \textit{``let her be in ancient times"} requires human intervention to prompt these models not to neglect elements like \textit{``replacing her contemporary attire with period-appropriate garments"}, in addition to \textit{``change the background to reflect an ancient era"}.
So, enhancing the self-reasoning capabilities is not only user-friendly, but also key to the advancement of next-generation intelligent AIGC systems.

% To advance self-reasoning proficiencies, a plausible approach might encompass substituting the CLIP model with the Large Language Model (LLM). Previous methods typically employ the CLIP text encoder to comprehend instructions. Nevertheless, As shown in Figure~\ref{}, the text encoder within the CLIP model predominantly concentrates on the linguistic components of the input, rather than the semantic structure of the sentence as a whole. This restricts its ability to carry out instruction following and reasoning tasks effectively.  On the contrary, the LLM model exhibits a significant proficiency in reasoning capabilities, suggesting prospective application in instruction-editing tasks.

Instruction reasoning for image editing necessitates not only the reliance on reasoning capability of LLM, but also demands the ability of comprehending the given image. 
For instance, when presented with the instruction \textit{``make it 50 years later"} for a variety of given images, the editing outcomes should be different. Accordingly, we employ a Multimodal Large Language Model (MLLM) instead of a singular large language model.

The potential of generative models aided by MLLM for reasoning-aware instruction editing is considerable. Nonetheless, existing datasets designated for instruction editing fails to fully unlock and exploit the inherent reasoning capabilities of the models. Thus,  we develope a comprehensive reasoning-attentive instruction editing dataset, comprising both image pairs and accompanying reasoning instructions. This dataset deviates from conventional datasets in several ways: 1) implicit instructions to further the model's reasoning capability, 2) an abundant of real images taken from fine-grained categories, and 3) increased variances between the input and the subsequently edited images, particularly at the geometric level.

Leveraging the proposed dataset, we introduce ReasonPix2Pix, a  intelligent image editing architecture. This innovative framework enhances the reasoning abilities of image editing and significantly boosts the quality of instructional editing. Our contribution can be summarized as follows:
\begin{itemize}[leftmargin=*]
\vspace{0.3em}
\itemsep0.3em
\item We propose ReasonPix2Pix, an instruction-based image editing framework with reasoning capabilities. Leveraging the power of the MLLM, ReasonPix2Pix demonstrates its intelligence in understanding human intent.
\item We develope a comprehensive reasoning-attentive instruction editing dataset, comprising both image pairs and accompanying reasoning instructions.
\item Our approach demonstrates not only superior performance in instruction editing tasks that do not necessitate reasoning, but also performs adequately in tasks necessitating reasoning.
\end{itemize}


\begin{figure}[h!]
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/pearl/in.jpg}
        \begin{center}
        \vspace{-2.5mm}
        \scriptsize Input
        \vspace{-1.5mm}
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/pearl/glass.jpg}
        \begin{center}
        \vspace{-2.5mm}
        \scriptsize Add a pair of sunglasses
        \vspace{-1.5mm}
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/pearl/prefer.jpg}
        \begin{center}
        \vspace{-2.5mm}
        \scriptsize she prefers face mask to sunglasses
        \vspace{-1.5mm}
        \end{center}
    \end{subfigure}%
    
    \caption{Previous method, InstructPix2Pix, is capable of tackling instruction 'add a pair of sunglasses, but it generates absolutely wrong result for the instruction 'she prefers face mask to sunglasses'.}
    \label{fig:pearl-mistake}
\end{figure}

\begin{comment}
\begin{figure}[h!]
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/gaki/in.jpg}
        \begin{center}
        \scriptsize Input
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/gaki/out.jpg}
        \begin{center}
        \scriptsize Output
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/gaki/out.jpg}
        \begin{center}
        \scriptsize Reasonable Output
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/apple/in.jpg}
        \begin{center}
        \scriptsize Input
        \end{center}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/apple/50.jpg}
        \begin{center}
        \scriptsize Output
        \end{center}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/apple/50-ours.jpg}
        \begin{center}
        \scriptsize Reasonable Output
        \end{center}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/statue/in.jpg}
        \begin{center}
        \scriptsize Input
        \end{center}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/statue/50.jpg}
        \begin{center}
        \scriptsize Output
        \end{center}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[t]{0.327\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/statue/50-ours.jpg}
        \begin{center}
        \scriptsize Output
        \end{center}
    \end{subfigure}%
    
    \caption{For the instruction 'make it 50 years later', previous methods can make a young woman to an old one, but cannot generate any results for fruit input (apple). In addition, when the input is a statue man, previous methods still make it old, which is wrong. The reasonable results shall be an old woman, a rotted fruit, and a broken statue respectively. Understanding of instruction is not a single-modal problem, the input image must be taken into consideration together. }
    \label{fig:50-years}
\end{figure}
\end{comment}

\begin{figure*}[pt]
   \begin{center}
   \includegraphics[width=1\linewidth]{./images/intro.pdf}
   \end{center}
   \caption{For the instruction 'make it 50 years later', previous methods can make a young woman to an old one, but cannot generate any results for fruit input (apple). In addition, when the input is a statue man, previous methods still make it old, which is wrong. The reasonable results may be an old woman, a rotted fruit, and a broken statue respectively. Understanding of instruction is not a single-modal problem, the input image must be taken into consideration together.}
   \label{fig:50-years}
\end{figure*}

==> sec/method.tex <==
\section{Methodology}
\label{sec:method}

Our objective is to perform image editing in accordance with human instructions, with a particular emphasis on reasoning instructions. Given an input image denoted as $x_{\text{input}}$ and a human instruction denoted as $c_{T}$, our model is designed to comprehend the explicit or implicit intents of human and subsequently generate the output image $x_{\text{edit}}$ that aligns with the provided instruction. To achieve this objective, we introduce ReasonPix2Pix (Section~\ref{sec:ReasonPix2Pix}), a model specifically tailored for instruction-based image editing with a focus on reasoning capabilities. ReasonPix2Pix comprises a multimodal large language model coupled with a diffusion model. In order to unlock and leverage the inherent reasoning capacities of the ReasonPix2Pix , we have curated an extensive reasoning-attentive instruction editing dataset (Section~\ref{sec:RISE}), which serves as the foundational training data for our model.

\subsection{ReasonPix2Pix}
\label{sec:ReasonPix2Pix}

The conventional instruction-editing model usually consists of a text encoder and a diffusion model.  The text encoder, typically adopting the CLIP text encoder, is responsible for extracting the salient features from the instruction to guide the subsequent image editing process. Simultaneously, the diffusion model accesses these extracted features and diffuses the noised input image to align it with the provided instruction. 

To enhance the active reasoning capability of the editing model, we integrate a Multimodal Large Language Model (MLLM) into the framework, as depicted in Figure~\ref{fig:method}. Diverging from previous methodologies that comprehend human intent solely through text, the MLLM enhances understanding by incorporating both the instruction and the input image. Formally, the instruction feature $h$ with human's intent can be formulated as
\begin{align}
\begin{aligned}
    h = & \;  \mathcal{F}(\vx_{input}, c_{T}),
\end{aligned}
\end{align}
where $\mathcal{F}$ is the MLLM. $h$ is the output hidden state of $\mathcal{F}$, containing the multimodal understanding of our instruction. 


\subsection{Instruction Editing Dataset with Reasoning}
\label{sec:RISE}


\begin{figure}[pt]
   \begin{center}
   \includegraphics[width=1\linewidth]{./images/p2p/sample.pdf}
   \end{center}
   \caption{One sample from InstructPix2Pix dataset. For each paired image, it contains 1) input image and input caption, 2) edited image and edited caption, and 3) instruction.}
   \label{fig:p2p-sample}
\end{figure}



\subsection{Preliminaries}
\paragraph{InstructPix2Pix Dataset} InstructPix2Pix~\misscite{} produces an important large-scale paired dataset to enable insturction-based image editing. Concretely, As shown in Figure~\ref{fig:p2p-sample}, it contains 1) Input Image $\vx_{input}$ and Input Caption $C_{input}$, 2) Edited Image $\vx_{edit}$ and Edited Caption $C_{edit}$, and 3) Text Instruction $I$. 

\paragraph{V3Det Dataset} \textcolor{blue}{[mllm may be better than V3Det]} V3Det~\misscite{} is a vast detection dataset with 13,204 categories, with well-annotated bounding boxes. The images appear to be realistic and complex. 

\subsection{Dataset Generation} \textcolor{blue}{[Method first: architecture, loss/training]}

\begin{table}[h]
    \centering
    \caption{Comparison of three parts in our dataset. The data source is listed here. Our generated data is noted as 'Generated'.}
    \begin{tabular}{l|ccc}
    \toprule
    &Input Image & Edited Image & Instruction \\
    \midrule
    Part I& InstructPix2Pix & InstructPix2Pix & Generated \\
    Part II & InstructPix2Pix & Generated & Generated\\
    Part III & V3Det & Generated & Generated\\
    
    \bottomrule
    \end{tabular}
    \label{tab:setup}
\end{table}

\begin{table*}[]
\centering
\caption{Comparison of different dataset. }
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|cc|c}
\toprule
Dataset & Real Image & Reasoning Instruction & Text Example  \\
\midrule
InstructPix2Pix~\cite{brooks2023instructpix2pix} & \XSolidBrush  & \XSolidBrush & \textit{Turn fruits to a cake}\\
MagicBrush~\cite{zhang2023magicbrush} & \Checkmark & \XSolidBrush  & \textit{Make him wear a hat}\\
ReasonPix2Pix (Ours) & \Checkmark & \Checkmark & \textit{The beautiful woman wants to walk in a more comfortable manner.} \\
\bottomrule
\end{tabular}
}
\label{tab:data-comp}
\end{table*}

Towards injecting reasoning ability to image editing model, we construct a comprehensive reasoning-attentive instruction editing dataset. 
% We compare it with previous datasets in Table~\ref{tab:data-comp}.

According to the generation procedure, our generated dataset can be divided into three parts. As shown in Table~\ref{tab:setup}, Part I take the original image pair in InstructPix2Pix, with our generated instruction to enable instruction reasoning, in Part II we start from the input image from InstructPix2Pix, generate our own edited image and instructions, and in Part III, we take more realistic images from V3Det, and generate edited images and instructions. 

\paragraph{Filtering} Though achieving great success in instruction-based image editing, InstructPix2Pix model suffers from various failure cases. One typical failure case is that the model is prone to output the original image, \ie conduct no editing. Delving into the dataset, we observe that a proportion of edited image is highly similar to the input image. Therefore, we need to filter this part of data first, we distinguish them by
\begin{equation}
    ||\vx_{input} - \vx_{edit}||_2^2 < \tau,
\end{equation}
where $\tau$ is the threshold value of the divergence between the input image and edited image. If $\tau$ is too small, the input image and edited image appear to be too similar, so this pair of data will be abandoned. $\tau$ can be a pre-defined value or rank value (\eg pick out the $10\%$ worst data). 

\paragraph{Part I: Reasoning Instruction generation} For this part of data, we take the input and edited image directly from original InstructPix2Pix Dataset. To equit the model with the reasoning ability to understand instructions, we need to convert existing instructions $I$ to reasoning instructions $I_{rea}$, which is indirect, but still accurate. We take the large-scale language model, GPT-3.5~\misscite{} (denoted as $G$) to generate our reasoning instruction. 
\begin{figure*}[htbp]
    \begin{subfigure}[t]{\linewidth}
        \includegraphics[width=\linewidth]{cvpr2024/images/gen2.pdf}
        
    \end{subfigure}%
    
    \caption{Reasoning Instruction Generation. We utilized GPT-3.5 to generate several candidate instuctions according to given input caption, edited caption and instruction in the original dataset. Then GPT-3.5 selects the best instruction from these candidate instructions.}
    \label{fig:gen}
\end{figure*}

\begin{figure*}[htbp]
    \begin{center}
        \includegraphics[width=\linewidth]{cvpr2024/images/part2-gen.pdf}
    \end{center}
    \caption{Image Editing and Reasoning Instruction Generation. If the input image has no caption, BLIP2 will give an image caption. Spacy extracts the candidate categories in the caption. Then, Grounding DINO locates the objects in the image. GPT-3.5 produces 1) selected category, 2) target category and 3) reasoning instruction. Finally, GLIGEN generates the edited image. }
    \label{fig:gen2}
\end{figure*}

As shown in Figure~\ref{fig:gen}, we take input caption, edited caption and original instruction from InstructPix2Pix dataset, inject them to GPT-3.5, and ask GPT-3.5 to generate cadidate instructions. 
\begin{equation}
    I_{gen} = G(P_{gen}(C_{input}, C_{edit}, I)),
\end{equation}
where $P_{gen}()$ is the generation prompt we design to project the input caption, edited caption and original instruction to a new instruction $I_{gen}$. With our prompt, the generated instruction should be 1) indirect, 2) in the similar effect with original instructions. For each input, we repeat this procedure for $n$ times to generate multiple candidate instructions $I_{gen}^0, ..., I_{gen}^n$. 

Then we again ask GPT-3.5 to distinguish the best instruction among them. 
\begin{equation}
    I_{reason} = G(P_{select}(I_{gen}^0, ..., I_{gen}^n)),
\end{equation}
where $P_{gen}()$ is the generation prompt we design to ask GPT model to select the most suitable instruction from $I_{gen}^0, ..., I_{gen}^n$. The selected instruction is $I_{reason}$ and it will serve as the reasoning instruction in Part I data. Therefore, the Part I data includes $\vx_{input}$, $\vx_{edit}$, and 3) $I_{reason}$. 
% The selected instruction serves as the new instruction in our dataset. 

\paragraph{Part II $\&$ III: Image Editing and Reasoning Instruction Generation} To further improve the model capability, we expand the dataset with other two parts of data. % These parts of data targets on enhance model's ability to tackle with more complex object replacement tasks and more realistic images. 
These parts of data not only enhance the reasoning ability of our model, but also aims at improving our model's capability of takcling more realistic image with fine-grained categories and more variances between the input and edited image. 

\begin{figure*}[pt]
   \begin{center}
   \includegraphics[width=1\linewidth]{./images/method.pdf}
   \end{center}
   \caption{Method Overview. Multi-modal LLava takes both input image and instruction. With a projection layer, the output hidden state is injected to the text model, and then serves as the condition information. With the condition supervision and original image, our method generates the edited image.  }
   \label{fig:method}
\end{figure*}

We take the original input images from InstructPix2Pix and V3Det. The former is the same with Part I but the latter contains abundant real image from large amounts of categories. As shown in Figure~\ref{fig:gen2}, since the images from V3Det have no captions, so we first generate a caption through BLIP2. For images from InstructPix2Pix, we take the original input caption directly. For simplicity, we denote the input image and caption as $\vx_{input}$ and $C_{input}$.

The caption is passed to a Spacy~\misscite{} model $S$, an advanced Natural Language Processing (NLP) model to recognize entities in sentences. Here we utilize it to extract the candidate categories,
\begin{equation}
    y_1, ..., y_i = S(C_{input}),
\end{equation}
where $S$ extracts $i$ candidate categories. For instance, in Figure~\ref{fig:gen2}, Spacy takes $i=2$ categories,
\ie butterfly and flower. 

With these categories, we can locate the corresponding object in the image by Grounding DINO~\misscite{}. 
\begin{equation}
    b_k = DINO(\vx_{input}, y_k),
\end{equation}
where $b_k$ is the bounding box of object belongs to category $y_k$ in image $\vx_{input}$.

Then we inject the caption and candidate categories to GPT-3.5. Here we design another prompt to ask GPT-3.5 to output 1) one selected category, 2) the target category we need to replace it to, and 3) the reasoning instruction.
\begin{equation}
    y_{select}, y', I_{reason} = G(P_{replace}(C_{input}, y_1, ..., y_i)),
\end{equation}
where $P_{replace}$ is the prompt we introduce. It takes input caption and candidate categories, and produces the selected category $y_{select}$, the target category $y'$ and the reasoning instruction. We will replace $y_{select}$ with $y'$.
For Figure~\ref{fig:gen2}, GPT selects butterfly and produces the target category bee, therefore, the butterfly will be transformed to bee. 

Finally, GLIGEN will conduct replace object from $y_{select}$ category to $y'$ category.
\begin{equation}
    \vx'_{edit} = GLIGEN(\vx_{input}, y_{select}, b_{select}, y'),
\end{equation}
where $\vx'_{edit}$ is the generated edited image, and $b_{select}$ is the bounding box of the object belongs to $y_{select}$. 
Through this procedure, we obtain paired image ($\vx_{input}$ and $\vx'_{edit}$) and instruction $I_{reason}$, forming Part II and Part III in our dataset. 



\subsection{Architecture} \textcolor{blue}{[Proposed Dataset following]}
Then we moved to the architecture of our method. The original stable diffusion model can be divided into two parts, the text model and the image generative model. The former convert text input to condition supervision information while the latter conduct image generation or editing. In this paper, to enhance the active reasoning capability of the editing model, we introduce Multimodal Large Language Model to the framework. As shown in Figure~\ref{fig:method}, we adopt a Multimodal LLM, LLava~\misscite{} in our method. Unlike previous methods that only take text information, it absorbs both the image and text instruction. So

\begin{align}
\begin{aligned}
    h_{out} = & \;  \mathcal{F}(\vx_{input}, c_{T}),
\end{aligned}
\end{align}

where $\mathcal{F}$ is the Multimodal LLM, it takes both input image $\vx_{input}$ and text instruction $c_T$ into consideration. $h_{llm}$ is the output hidden state of the model, containing the multimodal understanding of our instruction. 

To inject $h_{llm}$ to the text model in stable diffusion model seamlessly, we abandoned several layers in the text model $\mathcal{T}$ and project $h_{llm}$ to suitable dimension by a projection layer $\gamma$. Therefore, the text condition will be 
\begin{align}
\begin{aligned}
    c_{out} = \mathcal{T}(\gamma(h_{llm})),
\end{aligned}
\end{align}

Finally, the image generative model can edit the input image under the supervision of $c_{out}$.
\begin{align}
\begin{aligned}
    \vx_{out} = \mathcal{M}(\vx_{input}, c_{out}),
\end{aligned}
\end{align}
where $\mathcal{M}$ is the image model, and $\vx_{out}$ is the corresponding output. 

Considering the large amounts of parameters in LLM, we fixed it and apply a LoRA~\misscite{} when finetuning our model. We follow previous method to keep text model fixed when training stable diffusion. The other parts, including LoRA, projection layer and the image generative model are all finetuned end-to-end. 




